Higgs-boson plus Dijets: Higher-Order Matching for High-Energy Predictions

Several important processes and analyses at the LHC are sensitive to higher-order perturbative corrections beyond what can currently be calculated at fixed order. The formalism of High Energy Jets (HEJ) calculates the corrections systematically enhanced for a large ratio of the centre-of-mass energy to the transverse momentum of the observed jets. These effects are relevant in the analysis of e.g. Higgs-boson production in association with dijets within the cuts devised to enhance the contribution from Vector Boson Fusion (VBF). HEJ obtains an all-order approximation, based on logarithmic corrections which are matched to fixed-order results in the cases where these can be readily evaluated. In this paper we present an improved framework for the matching utilised in HEJ, which for merging of tree-level results is mathematically equivalent to the one used so far. However, by starting from events generated at fixed order and supplementing these with the all-order summation, it is computationally simpler to obtain matching to calculations of high multiplicity. We demonstrate that the impact of the higher-multiplicity matching on predictions is small for the gluon-fusion (GF) contribution of Higgs-boson production in association with dijets in the VBF-region, so perturbative stability against high-multiplicity matching has been achieved within HEJ. We match the improved HEJ prediction to the inclusive next-to-leading order (NLO) cross section and compare to pure NLO in the h->photon photon channel with standard VBF cuts.

==> intro.tex <==

\section{Introduction}
\label{sec:Introduction}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

